Comfetch: Federated Learning of Large Networks on Constrained Clients via Sketching

Federated learning (FL) is a popular paradigm for private and collaborative model training on the edge. In centralized FL, the parameters of a global architecture (such as a deep neural network) are maintained and distributed by a central server/controller to clients who transmit model updates (gradients) back to the server based on local optimization. While many efforts have focused on reducing the communication complexity of gradient transmission, the vast majority of compression-based algorithms assume that each participating client is able to download and train the current and full set of parameters, which may not be a practical assumption depending on the resource constraints of smaller clients such as mobile devices. In this work, we propose a simple yet effective novel algorithm, Comfetch, which allows clients to train large networks using reduced representations of the global architecture via the count sketch, which reduces local computational and memory costs along with bi-directional communication complexity. We provide a nonconvex convergence guarantee and experimentally demonstrate that it is possible to learn large models, such as a deep convolutional network, through federated training on their sketched counterparts. The resulting global models exhibit competitive test accuracy over CIFAR10/100 classification when compared against un-compressed model training.

==> figures/figs/figure-accuracy.tex <==
\begin{figure}[!htbp]
    \begin{minipage}[c]{0.49\textwidth}
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \resizebox{0.95\linewidth}{!}{
        \includegraphics[]{figures/output/output-figure0.pdf}
        }
        \caption{\small{Accuracy vs Compression}}
        \label{fig:subfig8}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\textwidth}
    \centering
        \resizebox{0.95\linewidth}{!}{
        \includegraphics[]{figures/output/output-figure1.pdf}
        }
        \caption{\small{Accuracy vs Top-$k$ Ratio}}   
        \label{fig:subfig9}
    \end{subfigure}
    \end{minipage}
    \hfill
\begin{minipage}[c]{0.49\textwidth}
\caption{\footnotesize{Test accuracy achieved on CIFAR-10 classification. In \textbf{(a)}, we emphasize that \textbf{under the same communication compression $\mathsf{CR}$ (the horizontal axis),  the reported performance achieved by \texttt{Comfetch} requires $1/\mathsf{CR}$ times smaller client memory footprint than \texttt{FetchSGD}.} \texttt{FetchSGD} only compresses the network weights during communication, but each client still needs to decompress the entire network locally to perform training. So our constructions of the baselines are inherently advantaged against our \texttt{Comfetch}.
%``Uncompressed'' is the simple baseline where no compression is applied during training. 
% We implement \texttt{FetchSGD} and \texttt{FedAvg} following \citet{rothchild2020fetchsgd}.
}}\label{fig:CIFAR}
\end{minipage}
\vspace{-2em}
\end{figure}

==> figures/figs/figure-mlni.tex <==
\begin{figure}[!h]
    \centering
   \begin{subfigure}[b]{0.23\textwidth}
    \centering
        \resizebox{0.99\linewidth}{!}{
        \includegraphics[]{figures/output/output-figure8.pdf}
        }
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
    \centering
        \resizebox{0.99\linewidth}{!}{
        \includegraphics[]{figures/output/output-figure9.pdf}
        }
    \end{subfigure}
     \vspace{-0.8em}
    \caption{\footnotesize{Effects of the number of sketches used on part of speech taggings for MNLI~\cite{williams2017broad} sentences. We test in-layer recovery by taking the median of the result of multiple unsketches (left), and varying the number of clients (right). We find that 1) using multiple sketches to perform in-layer recovery improves accuracy, and 2) the performance of our algorithm does not significantly change with the number of sketches.}}
    \label{fig:varying-number-sketches-mnli}
\end{figure}

==> figures/figs/figure-num-sketch-test.tex <==
\begin{figure}[!ht]
\vspace{-1em}
    % \begin{subfigure}[b]{0.23\textwidth}
    % \centering
    %     \resizebox{0.99\linewidth}{!}{
    %     {\input{manuscript/figures/plots/CIFAR_test_1}}
    %     }
    %     \caption{Accuracy using 1 sketch}   
    % \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
    \centering
        \resizebox{0.99\linewidth}{!}{
        \includegraphics[]{figures/output/output-figure6.pdf}
        }
        \caption{Accuracy using 3 sketches}   
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
    \centering
        \resizebox{0.99\linewidth}{!}{
        \includegraphics[]{figures/output/output-figure7.pdf}
        }
        \caption{Accuracy using 5 sketches}   
    \end{subfigure}
    % \begin{subfigure}[b]{0.23\textwidth}
    % \caption{\small{Effects of the number of sketches used on CIFAR-10 classification. We send $N$ different sketches to the clients at each iteration of training. Our results suggest that performance does not degrade even when only 1 sketch is used across all clients, suggesting that in practice we could avoid sending multiple sketches to reduce bandwidth and memory costs while maintaining training robustness.}}
    % \label{fig:varying-number-sketches-cifar10}
    % \end{subfigure}
    \vspace{-0.5em}
    \caption{\footnotesize{Effects of the number of sketches used on CIFAR-10 classification. We send $N$ different sketches to the clients at each iteration of training. We observe that performance does not degrade even when only 1 sketch is used across all clients, suggesting that in practice we could avoid sending multiple sketches to reduce bandwidth and memory costs while maintaining training robustness.}}
    \label{fig:varying-number-sketches-cifar10}
\end{figure}

==> figures/figs/figure-num-sketch-train.tex <==
\begin{figure}[!htbp]
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \resizebox{0.99\linewidth}{!}{
        {\input{manuscript/figures/plots/CIFAR_train_1}}
        }
        \caption{Train Accuracy using 1 sketches}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \resizebox{0.99\linewidth}{!}{
        {\input{manuscript/figures/plots/CIFAR_train_3}}
        }
        \caption{Train Accuracy using 3 sketches}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \resizebox{0.99\linewidth}{!}{
        {\input{manuscript/figures/plots/CIFAR_train_5}}
        }
        \caption{Train Accuracy using 5 sketches}
    \end{subfigure}
\end{figure}

==> figures/imgs/count_sketch.tex <==
% Count Sketch Intuition Diagram

\begin{figure} 
  \includegraphics[width=\textwidth]{manuscript/figures/imgs/count_sketch.png}
\label{count_sketch}
\end{figure}

==> figures/imgs/fed_diagram.tex <==
% Federated Learning Aggregation Model Diagram
\begin{figure}[!htbp]%[20]{r}{0.5\textwidth}
%\vspace{-0.5em}
  \begin{center}
    \includegraphics[width=0.35\textwidth]{figures/imgs/fed_learning.pdf}
  \end{center}
%   \vspace{-0.5em}
  \caption{\footnotesize{\texttt{Comfetch} Communication. A high-level depiction of data being sent over the edge in \texttt{Comfetch}. The server communicates sketch key pairs to the client and the client uploads local gradients with respect to the sketched weights.}\label{fed_learning}}
%  \vspace{-1em}
\end{figure}

==> figures/updated-figs/cifar-pruning-comparison.tex <==
\begin{figure}[!htbp]
   \centering
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \resizebox{0.99\linewidth}{!}{
        \includegraphics[]{figures/updated-figs/cifar10-weight-prune-comparison-iid.pdf}
        }
        \caption{\small{CIFAR-10 Test Accuracy}}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.23\textwidth}
    \centering
        \resizebox{0.99\linewidth}{!}{
        \includegraphics[]{figures/updated-figs/cifar100-weight-prune-comparison-iid.pdf}
        }
        \caption{\small{CIFAR-100 Test Accuracy}}
    \end{subfigure}
     \vspace{-0.5em}
    \caption{\footnotesize{Test accuracy convergence of \texttt{Comfetch} compared to weighted pruning under varying compression rates. In these experiments, only a single sketch is used and the datasets are IID.}}
    \label{fig:convergence-effect-pruning}
\end{figure}

==> figures/updated-tables/cifar10-prune-comparison.tex <==
\begin{table}[!htbp]
\begin{minipage}[c]{0.49\textwidth}
\label{cnncompressiontable-prune}
    \centering
    \resizebox{0.99      \textwidth}{!}{\scriptsize{\begin{tabular}
    {c>{\centering\arraybackslash}p{0.25\textwidth}>{\centering\arraybackslash}p{0.25\textwidth}>{\centering\arraybackslash}p{0.25\textwidth}}
        \toprule
        \scriptsize{Method} &  \scriptsize{Compression Rate}  & \scriptsize{Test Accuracy (\%)}  \\
        \midrule
        \texttt{Weighted Pruning} & 90\%  & \textbf{79.02} \\
        \texttt{Comfetch} & 90\% &   76.53 \\
        \midrule
        \texttt{Weighted Pruning} & 75\% &  82.32 \\
        \texttt{Comfetch} & 75\% & \textbf{82.85} \\
        \midrule
        \texttt{Weighted Pruning} & 50\%  &  \textbf{84.56} \\
        \texttt{Comfetch} & 50\% & 84.42 \\
        \bottomrule
    \end{tabular}}}
    \end{minipage}
    \hfill
\begin{minipage}[c]{0.49\textwidth}
    \caption{\footnotesize{Average test accuracy over three random runs for 10 clients classifying CIFAR-10 \cite{cifar10} using ResNet18. We compare a weighted pruning approach with \texttt{Comfetch}. %\texttt{Comfetch} maintains a large and powerful global model under communication compression and client memory compression, whereas the baseline requires the global model to be smaller to obtain the same communication and client memory efficiency. 
    %Since \texttt{FedAvg} and \texttt{FetchSGD} cannot achieve any memory compression by design, we reduce the global network layer width to achieve a de facto reduction in memory. While \texttt{FetchSGD} focuses on bandwidth compression, we obtain its best-case performance by setting the bandwidth compression ratio as 1. The results indicate that our methods achieve competitive performance when the bandwidth and client memory are limited.
    }  }
    \label{tab:prune-cifar10}
    \end{minipage}
\end{table}


==> figures/updated-tables/cifar100-prune-comparison.tex <==
\begin{table}[!htbp]
\begin{minipage}[c]{0.49\textwidth}
\label{cifar100compressiontable}
    \centering
    \resizebox{0.99      \textwidth}{!}{\scriptsize{\begin{tabular}
    {c>{\centering\arraybackslash}p{0.25\textwidth}>{\centering\arraybackslash}p{0.25\textwidth}>{\centering\arraybackslash}p{0.25\textwidth}}
        \toprule
        \scriptsize{Method} &  \scriptsize{Compression Rate}  & \scriptsize{Test Accuracy (\%)}  \\
        \midrule
        \texttt{Weighted Pruning} & 90\%  & \textbf{48.35} \\
        \texttt{Comfetch} & 90\% &   43.80 \\
        \midrule
        \texttt{Weighted Pruning} & 75\% &  52.08 \\
        \texttt{Comfetch} & 75\% & \textbf{52.25} \\
        \midrule
        \texttt{Weighted Pruning} & 50\%  &  \textbf{55.03} \\
        \texttt{Comfetch} & 50\% & 54.76 \\
        \bottomrule
    \end{tabular}}}
    \end{minipage}
    \hfill
\begin{minipage}[c]{0.49\textwidth}
    \caption{\footnotesize{Average test accuracy over three random runs for 10 clients classifying CIFAR-100 \cite{cifar10} using ResNet18. We compare a weighted pruning approach with \texttt{Comfetch}. %\texttt{Comfetch} maintains a large and powerful global model under communication compression and client memory compression, whereas the baseline requires the global model to be smaller to obtain the same communication and client memory efficiency. 
    %Since \texttt{FedAvg} and \texttt{FetchSGD} cannot achieve any memory compression by design, we reduce the global network layer width to achieve a de facto reduction in memory. While \texttt{FetchSGD} focuses on bandwidth compression, we obtain its best-case performance by setting the bandwidth compression ratio as 1. The results indicate that our methods achieve competitive performance when the bandwidth and client memory are limited.
    }  }
    \label{tab:prune-cifar100}
    \end{minipage}
\end{table}
